Inference of Shape Expression Schemas Typed RDF Graphs

We consider the problem of constructing a Shape Expression Schema (ShEx) that describes the structure of a given input RDF graph. We employ the framework of grammatical inference, where the objective is to find an inference algorithm that is both sound i.e., always producing a schema that validates the input RDF graph, and complete i.e., able to produce any schema, within a given class of schemas, provided that a sufficiently informative input graph is presented. We study the case where the input graph is typed i.e., every node is given with its types. We limit our attention to a practical fragment ShEx0 of Shape Expressions Schemas that has an equivalent graphical representation in the form of shape graphs. We investigate the problem of constructing a canonical representative of a given shape graph. Finally, we present a sound and complete algorithm for shape graphs thus showing that ShEx0 is learnable from typed graphs.

==> hybrid.tex <==
\section{Hybrid approach}
\label{sec:hybrid}
In this section we extend the simulation-based approach with a modest dose
of context information: we consider the paths of ancestors up nodes can be distinguished by their  of ancestor nodes. The purpose of this extension is to show how we can carefully combine the previous two
approaches to reach a trade-off between their ability to introduce recursive
types and the inability to identify subtypes while avoiding producing schemas
that are overfitted and potentially too verbose.

We illustrate the proposed $\hybridlearner$ algorithm in
Figure~\ref{fig:hybrid-learner} on the graph $G_0$ from
Figure~\ref{fig:example}.
\begin{figure}[htb]
  \centering
  \begin{tikzpicture}[>=latex]%, scale=1.5, transform shape]
    \footnotesize
%    \path[use as bounding box] (-1.25,0.75) rectangle (9,-3.125);
    % \begin{scope}[xshift=-5cm,yshift=-0.5cm,bend angle=15]
    % \node at (0,1.65) {$G_0^\circ$}; 
    % % \node (bug3) at (0,0) {\tt b${}_3$};
    % % \node (bug1) at (1,1) {\tt b${}_1$};
    % % \node (bug4) at (2.5,0) {\tt b${}_4$};
    % % \node (bug2) at (3.0125,1) {\tt b${}_2$};

    % % \node (user1) at (0,-1.25) {\tt u${}_1$};
    % % \node (user2) at (3.125,-1.25) {\tt u${}_2$};
    % % \node (emp1) at (1.75,-1.25) {\tt e${}_1$};

    % % \node (s) at (1,-2.5) {$\str$};

    % \node (bug3) at (0,0) {\tt b${}_3$};
    % \node (bug1) at (1,1) {\tt b${}_1$};
    % \node (bug4) at (2.5,0) {\tt b${}_4$};
    % \node (bug2) at (3.0125,1) {\tt b${}_2$};

    % \node (user1) at (0,-1.25) {\tt u${}_1$};
    % \node (user2) at (3.125,-1.25) {\tt u${}_2$};
    % \node (emp1v) at (1.5,-.5) {\tt e${}_1^\mathtt{v}$};
    % \node (emp1s) at (1.75,-1.25) {\tt e${}_1^\mathtt{s}$};

    % \node (s) at (1,-2.5) {$\str$};
    % \draw (bug1) edge[->,bend left] node[above,sloped] {\tt r} (bug4);
    % \draw (bug1) edge[->,bend right] node[above,sloped] {\tt r} (bug3);
    % \draw (bug1) edge[->,bend left] node[above,sloped] {\tt s} (user1);
    % \draw (bug1) edge[->,bend left] node[above,sloped] {\tt v} (emp1v);

    % \draw[bend angle=05] (bug2) edge[->,bend right] node[above,sloped] {\tt r} (bug4);
    % \draw[bend angle=05] (bug2) edge[->,bend left] node[above=-1pt,sloped] {\tt s} (user2);

    % \draw (bug3) edge[->,bend right] node[above,sloped] {\tt s} (user1);

    % \draw[bend angle=05] (bug4) edge[->,bend right] node[above=-1pt,sloped] {\tt s} (emp1s);

    % \draw[bend angle=10] (bug1) edge[->, bend right] node[below=-1pt,sloped,pos=0.6] {\tt d} (s);
    % \draw (bug2) edge[->, bend left,in=137,out=20] node[above=-1pt,sloped,pos=0.35] {\tt d} (s);
    % \draw (bug3) edge[->, bend right,out=-80,in=-110] node[below=-1pt,sloped] {\tt d} (s);
    % \draw (bug4) edge[->, bend left,in=140] node[above=-1pt,sloped,pos=0.45] {\tt d} (s);
    % \draw (user1) edge[->, bend right] node[above,sloped] {\tt n} (s);
    % \draw[bend angle=20] (user2) edge[->,bend left] node[above=-1pt,sloped,pos=0.3] {\tt n} (s);
    % \draw[bend angle=35] (user2) edge[->,bend left] node[below,sloped] {\tt e} (s);
    % \draw[bend angle=10] (emp1s) edge[->,bend right] node[below=-1pt,sloped,pos=0.4] {\tt n} (s);
    % \draw[bend angle=25] (emp1s) edge[->,bend left] node[below=-2pt,sloped,pos=0.35] {\tt e} (s);    
    % \draw[bend angle=20] (emp1v) edge[->,bend right] node[above=-1pt,sloped,pos=0.3] {\tt n} (s);
    % \draw[bend angle=10] (emp1v) edge[->,bend left,in=187] node[below=-2pt,sloped,pos=0.15] {\tt e} (s);    
    % \end{scope}

    \begin{scope}[xshift=-0.5cm,yshift=-0.5cm,bend angle=15,
        every edge/.style={draw,gray}]
    \node at (0,1.5) {$G_0^\MANY$};
    \node (bug3) at (0,0) {\tt b${}_3$};
    \node (bug1) at (1,1) {\tt b${}_1$};
    \node (bug4) at (2.5,0) {\tt b${}_4$};
    \node (bug2) at (3.0125,1) {\tt b${}_2$};

    \node (user1) at (0,-1.25) {\tt u${}_1$};
    \node (user2) at (3.125,-1.25) {\tt u${}_2$};
    \node (emp1v) at (1.5,-.5) {\tt e${}_1^\mathtt{v}$};
    \node (emp1s) at (1.75,-1.25) {\tt e${}_1^\mathtt{s}$};

    \node (s) at (1,-2.5) {$\str$};
    \draw (bug1) edge[->,bend left] node[above,sloped] {\tt r\MANY} (bug4);
    \draw (bug1) edge[->,bend right] node[above,sloped] {\tt r\MANY} (bug3);
    \draw (bug1) edge[->,bend left] node[above,sloped] {\tt s\MANY} (user1);
    \draw (bug1) edge[->,bend left] node[above,sloped] {\tt v\MANY} (emp1v);

    \draw[bend angle=05] (bug2) edge[->,bend right] node[above,sloped] {\tt r\MANY} (bug4);
    \draw[bend angle=05] (bug2) edge[->,bend left] node[above=-1pt,sloped] {\tt s\MANY} (user2);

    \draw (bug3) edge[->,bend right] node[above,sloped] {\tt s\MANY} (user1);

    \draw[bend angle=05] (bug4) edge[->,bend right] node[above=-1pt,sloped] {\tt s\MANY} (emp1s);

    \draw[bend angle=10] (bug1) edge[->, bend right] node[below=-1pt,sloped,pos=0.6] {\tt d\MANY} (s);
    \draw (bug2) edge[->, bend left,in=137,out=20] node[above=-1pt,sloped,pos=0.35] {\tt d\MANY} (s);
    \draw (bug3) edge[->, bend right,out=-80,in=-110] node[below=-1pt,sloped] {\tt d\MANY} (s);
    \draw (bug4) edge[->, bend left,in=140] node[above=-1pt,sloped,pos=0.45] {\tt d\MANY} (s);
    \draw (user1) edge[->, bend right] node[above,sloped] {\tt n\MANY} (s);
    \draw[bend angle=20] (user2) edge[->,bend left] node[above=-1pt,sloped,pos=0.3] {\tt n\MANY} (s);
    \draw[bend angle=35] (user2) edge[->,bend left] node[below,sloped] {\tt e\MANY} (s);
    \draw[bend angle=10] (emp1s) edge[->,bend right] node[below=-1pt,sloped,pos=0.4] {\tt n\MANY} (s);
    \draw[bend angle=25] (emp1s) edge[->,bend left] node[below=-2pt,sloped,pos=0.35] {\tt e\MANY} (s);    
    \draw[bend angle=20] (emp1v) edge[->,bend right] node[above=-1pt,sloped,pos=0.3] {\tt n\MANY} (s);
    \draw[bend angle=10] (emp1v) edge[->,bend left,in=187] node[below=-2pt,sloped,pos=0.15] {\tt e\MANY} (s);    
    \end{scope}
    \begin{scope}[xshift=5cm,yshift=-0.5cm,bend angle=15,
    every edge/.style={draw,gray}]
    \node at (0,1.5) {$H_0=\uncouple(G_0^\MANY,1)$};
    \node (bug3) at (-1,0) {\tt b${}_3$};
    \node (bug1) at (1,1) {\tt b${}_1$};
    \node (bug4) at (2.5,.4) {\tt b${}_1$rb${}_4$};
    \node (bug4b2) at (3.2,-.4) {\tt b${}_2$rb${}_4$};
     \node (bug2) at (4,.5) {\tt b${}_2$};

    \node (user1) at (0,-.7) {\tt b${}_1$su${}_1$};
    \node (user1b3) at (-.7,-1.35) {\tt b${}_3$su${}_1$};
    \node (user2) at (3.5,-1.85) {\tt u${}_2$};
    \node (emp1v) at (1.5,-.5) {\tt e${}_1^\mathtt{v}$};
    \node (emp1s) at (2.3,-1.1) {\tt e${}_1^\mathtt{s}$};

    \node (s) at (1,-2.5) {$\str$};
    \draw (bug1) edge[->,bend left] node[above,sloped] {\tt r\MANY} (bug4);
    \draw (bug1) edge[->,bend right] node[above,sloped] {\tt r\MANY} (bug3);
    \draw (bug1) edge[->,bend right] node[above,sloped] {\tt s\MANY} (user1);
    \draw (bug1) edge[->,bend left] node[above,sloped] {\tt v\MANY} (emp1v);

    \draw[bend angle=05] (bug2) edge[->,bend right] node[above,sloped] {\tt r\MANY} (bug4b2);
    \draw[bend angle=05] (bug2) edge[->,bend left] node[below=-1pt,sloped] {\tt s\MANY} (user2);

    \draw (bug3) edge[->,bend right] node[above,sloped] {\tt s\MANY} (user1b3);

    \draw[bend angle=05] (bug4) edge[->,bend right] node[above=-1pt,sloped] {\tt s\MANY} (emp1s);
    \draw[bend angle=05] (bug4b2) edge[->,bend right] node[above=-1pt,sloped] {\tt s\MANY} (emp1s);

    \draw[bend angle=10] (bug1) edge[->, bend right] node[below=-1pt,sloped,pos=0.6] {\tt d\MANY} (s);
    \draw (bug2) edge[->, bend left,in=137,out=20] node[above=-1pt,sloped,pos=0.35] {\tt d\MANY} (s);
    \draw (bug3) edge[->, bend right,out=-80,in=-110] node[below=-1pt,sloped] {\tt d\MANY} (s);
    \draw (bug4) edge[->, bend right,in=170] node[above=-1pt,sloped,pos=0.1] {\tt d\MANY} (s);
    \draw (bug4b2) edge[->, bend left,in=140] node[above=-1pt,sloped,pos=0.2] {\tt d\MANY} (s);
    \draw (user1) edge[->, bend right] node[above,sloped] {\tt n\MANY} (s);
    \draw (user1b3) edge[->, bend right] node[above,sloped] {\tt n\MANY} (s);
    \draw[bend angle=20] (user2) edge[->,bend left] node[above=-1pt,sloped,pos=0.3] {\tt n\MANY} (s);
    \draw[bend angle=35] (user2) edge[->,bend left] node[below,sloped] {\tt e\MANY} (s);
    \draw[bend angle=10] (emp1s) edge[->,bend right] node[below=-1pt,sloped,pos=0.4] {\tt n\MANY} (s);
    \draw[bend angle=25] (emp1s) edge[->,bend left] node[below=-2pt,sloped,pos=0.35] {\tt e\MANY} (s);    
    \draw[bend angle=20] (emp1v) edge[->,bend right] node[above=-1pt,sloped,pos=0.3] {\tt n\MANY} (s);
    \draw[bend angle=10] (emp1v) edge[->,bend left,in=187] node[below=-2pt,sloped,pos=0.15] {\tt e\MANY} (s);    
    \end{scope}
    
%    \begin{scope}[xshift=10cm,yshift=0cm]
%    \node[below right,text width=2cm] (n) at (0,0.5) {\renewcommand{\arraystretch}{1.4}
%    In $G_O^\MANY$\\ 
%    ($\dominate$ over descendants):\\
%  $  \begin{array}{l}
%    b_3\dominate b_4\dominate b_2\\
%    b_3\dominate b_1\\
%    u_1\dominate u_2\equiv e_1^s\equiv e_1^v
%    \end{array}$};               2            2 0
%    \node[below right,text width=2cm] (n) at (0,-2.2) {\renewcommand{\arraystretch}{1.4}
%    In $H_0$:\\
%    ($\dominate$ over descendants and ancestors -perhaps better to draw  a DAG of dominance classes):\\
%  $  \begin{array}{l}
%    b_2rb_4\dominate b_2\\
%    b_3\dominate b_1rb_4\dominate b_2\\
%    b_3su_1\dominate b_1su_1\\
%    b_3su_1\dominate e_1^s\dominate u_2\\
%b_3\dominate b_1\\
%        \end{array}$\\
%        Our result for $\mathsf{reduce}$ assumes we merge: \\
%        b${}_3$ into b${}_2$\\
%        b${}_3$su${}_1$ into $u_2$\\
%         };
%    \end{scope}
    
    \begin{scope}[xshift=-2cm,yshift=-5cm, 
    every edge/.style={draw,blue},
    nd/.style={draw},
    dm/.style={->}
   ]
    \node at (1,1) {$\dominate$ in $G_0^\MANY$};
    \node[nd] (bug1) at (2,0) {\tt b${}_1$};
    \node[nd](bug2) at (3,0) {\tt b${}_2$};
    \node[nd] (bug4) at (2.5,-1) {\tt b${}_4$};
    \node[nd] (bug3) at (2,-2) {\tt b${}_3$};
    \node[nd] (emp1v) at (.5,0) {\tt e${}_1^\mathtt{v}\equiv e{}_1^\mathtt{s}\equiv u_2$};
    \node[nd] (user1) at (.5,-2) {\tt u${}_1$};
    \draw[dm] 
   (user1) edge (emp1v)
   (bug3) edge (bug1)
   (bug3) edge (bug4)
   (bug4) edge (bug2)
   ;
      
    \end{scope}
 \begin{scope}[xshift=-2cm,yshift=-9cm, 
    every edge/.style={draw,blue},
    nd/.style={draw},
    dm/.style={->},
    ns/.style={dashed}
    ]
    \node at (1,1) {$\dominate_h$ in $H_0$};
    \node[nd] (user1-1) at (1,0) {\tt b${}_1$su${}_1$};
    \node[nd] (bug1) at (2,0) {\tt b${}_1$};
    \node[nd](bug2) at (3,0) {\tt b${}_2$};
    \node[nd] (bug4-1) at (2.75,-1) {\tt b${}_1$rb${}_4$};
    \node[nd] (bug4-2) at (3.75,-1) {\tt b${}_2$rb${}_4$};
    \node[nd] (bug3) at (2,-2) {\tt b${}_3$};
    \node[nd] (user2) at (0,0) {\tt  u${}_2$};
    \node[nd] (user1-3) at (.5,-2) {\tt b${}_3$su${}_1$};
	 \node[nd] (emp1s) at (0,-1) {\tt e${}_1^\mathtt{s}$};
	 \node[nd] (emp1v) at (3.75,0) {\tt e${}_1^\mathtt{v}$};
    \draw[dm] 
%   (bug4-1) edge (bug2)
%   (bug4-2) edge (bug2)
   (bug3) edge (bug4-1)
%   (bug3) edge (bug1)
   (user1-3) edge (user1-1)
   (user1-3) edge (emp1s)
%   (emp1s) edge (user2)
   ;
    \end{scope}
    
    \begin{scope}[xshift=4cm,yshift=-5cm, 
    every edge/.style={draw,gray}]
    \node at (-1.5,1) {$\mathsf{reduce}(H,\mathord{\dominate})$ TODO FIX};
    \node (mb) at (0,0.5) {\tt b${}_1$};
    \node (b) at (0,-0.5) {\tt b${}_2$};
    \node (u) at (-.5,-1.75) {\tt u${}_2$};
    \node (bu) at (1.5,-1.75) {\tt b${}_1$su${}_1$};
    \node (e) at (0.5,-1.75) {\tt e${}_1^\mathtt{v}$};
    \node (s) at (0,-3) {$\mathsf{str}$};

    \draw[bend angle=15] (u) edge[->,bend right] node[below=-1pt,sloped,pos=0.4] {\tt n\MANY}  (s);
    \draw[bend angle=15] (u) edge[->,bend left] node[above=-1pt,sloped,pos=0.15] {\tt e\MANY} (s);
    \draw[bend angle=15] (e) edge[->,bend right] node[above=-2pt,sloped,pos=0.2] {\tt n\MANY}  (s);
    \draw[bend angle=15] (e) edge[->,bend left] node[below=-1pt,sloped] {\tt e\MANY} (s);
    \draw[bend angle=15] (bu) edge[->,bend left] node[below=-1pt,sloped] {\tt n\MANY} (s);
   
    \draw (mb) edge[->] node[above,sloped] {\tt r\MANY}  (b);
    \draw (mb) edge[->,bend left] node[above,sloped] {\tt v\MANY}  (e);
%    \draw (mb) edge[->,out=50,in=130,looseness=1,loop] node[above,sloped] {\tt r\MANY}  (mb);
    \draw (mb) edge[->,bend left] node[above,sloped] {\tt s\MANY} (bu);
    \draw[bend angle=15] (b) edge[->,bend right] node[above=-1pt,sloped,pos=0.3] {\tt s\MANY} (u);
    \draw (b) edge[->,out=110,in=160,looseness=.5,loop] node[above,sloped] {\tt r\MANY}  (b);
    \draw (b) edge[->] node[above,sloped,pos=0.35] {\tt d\MANY} (s);
    \draw[bend right] (mb) edge[->,out=-80,in=250,looseness=1.3] node[below,sloped] {\tt d\MANY} (s);
    \end{scope}
    \begin{scope}[xshift=8cm,yshift=-5cm,
            every edge/.style={draw,gray}]
    \node at (-.9,0.75) {$H_2$  TODO FIX};
    \node (mb) at (0,0.5) {\tt b${}_1$};
    \node (b) at (0,-0.5) {\tt b${}_2$};
    \node (u) at (-.5,-1.75) {\tt u${}_2$};
    \node (e) at (0.5,-1.75) {\tt e${}_1^\mathtt{v}$};
    \node (bu) at (1.5,-1.75) {\tt b${}_1$su${}_1$};
    \node (s) at (0,-3) {$\mathsf{str}$};

    \draw[bend angle=15] (u) edge[->,bend right] node[below=-1pt,sloped,pos=0.4] {\tt n}  (s);
    \draw[bend angle=15] (u) edge[->,bend left] node[above=-1pt,sloped,pos=0.15] {\tt e\MAYBE} (s);
    \draw[bend angle=15] (e) edge[->,bend right] node[above=-2pt,sloped,pos=0.2] {\tt n}  (s);
    \draw[bend angle=15] (e) edge[->,bend left] node[below=-1pt,sloped] {\tt e\color{red!70!black}\bfseries \MAYBE} (s);
    \draw[bend angle=15] (bu) edge[->,bend left] node[above=-2pt,sloped,pos=0.2] {\tt n}  (s);
   
    \draw (mb) edge[->] node[above,sloped] {\tt r\MANY}  (b);
    \draw (mb) edge[->,bend left] node[above,sloped] {\tt v\MAYBE}  (e);
    \draw (mb) edge[->,bend left] node[above,sloped] {\tt s}  (bu);
    \draw[bend angle=15] (b) edge[->,bend right] node[above=-1pt,sloped,pos=0.3] {\tt s} (u);
    \draw (b) edge[->,out=110,in=160,looseness=.5,loop] node[above,sloped] {\tt r\MANY}  (b);
    \draw (b) edge[->] node[above,sloped,pos=0.35] {\tt d} (s);
    \draw[bend right] (mb) edge[->,out=-70,in=240] node[below,sloped] {\tt d} (s);
    \end{scope}
  \end{tikzpicture}
  \caption{$\hybridlearner$: uncoupling and generalization
    $G_0^\MANY$, reduction $G_0^R$, and specialization $H_2$.}
  \label{fig:hybrid-learner}
\end{figure}


\begin{algorithm}
  \flushleft
\caption{\label{alg:hybrid-infer}Outline of  the inference algorithm for \HybShExZero.}
\ALGORITHM $\mathsf{\hybridlearner}(G)$\\
\INPUT $G=(N_G,E_G)$ a simple graph\\
\PARAM $M$ a proper set of intervals, $k$ integer\\
\OUTPUT $K\in\SinShExZero(M)$ inferred schema\\[5pt]
\BEGIN\\
\LN $G_\MANY\colonequals\mathsf{generalize}(G)$ \\
\LN $H_0\colonequals\uncouple(G_\MANY,k)$\\
\LN $H\colonequals\mathsf{reduce}(H_0,\mathord{\dominate}_h)$\\
\LN $\mathit{typing}\colonequals\textit{induced-embedding}(G,H)$\\
\LN $K\colonequals\mathsf{specialize}_M(H,G,\mathit{typing})$\\
\LN \RETURN $K$\\
\END\\

\PROCEDURE $\mathsf{uncouple}(G,k)$\\
\LN $N_H=\emptyset$\\
\LN \FOR $n \in N_G$ \DO\\
\LN \TAB $N_H\colonequals N_H\cup\AncPaths_G(n,k)$\\
\LN $E_H=\emptyset$\\
\LN \FOR $\pi \cdot a\cdot n_0\in N_H$ \DO\\
\LN \TAB \FOR $\pi'\in N_H$ \DO\\
\LN \TAB \TAB \IF $\pi\sqsubseteq\pi'$ \THEN\\
\LN \TAB \TAB \TAB $E_H\colonequals E_H \cup \{(\pi',a,\pi)\}$\\
\LN \RETURN $(N_H,E_H)$\\
\END \\[5pt]
\end{algorithm} 

 A \emph{path} $\pi$ in $G$ is a sequence $n_0\cdot a_1\cdot n_1\dots a_k\cdot n_k$ such that
$(n_0,a_1,n_1),(n_1,a_2,n_2),\ldots,(n_{k-1},a_k,n_k)\in
E_G$. The \emph{length} of $\pi$ is $k$, its \emph{source} is
$\source(\pi)=n_0$, its \emph{target} is $\target(\pi)=n_k$. As a special case we consider paths of length $0$ defined as a single node $n_0\in N_G$.
We denote by $\sqsubseteq$ we denote the standard prefix relation.
An \emph{ancestor path} of $n$ is any path that terminates in $n$ and by $\AncPaths_G(n,k)$ we denote the set all (suffix-) maximal ancestor paths of $n$ in $G$ of length at most $k$. This means we take all maximal suffixes of paths of length at most $k$, or equivalently all paths of length at most $k$ that cannot be completed into a longer such path by adding a prefix. (TODO check terminology, clarify if needs be)

The uncoupling of a graph $G$ to depth $k$, $\uncouple(G,k)$, is defined through the following construction: every node $n$ is replaced with one copy per path in $\AncPaths_G(n,k)$, then the incoming edges are re-distributed as explained in the algorithm.

Given a path $\pi=n_0\cdot a_0\dots n_i$ in $G$, we denote by $\mathsf{last}(\pi)$ the last node in the path, namely $n_i$. 
%Given a path $\pi'=u_0\cdot b_0\cdot  u_1\dots u_k$ in $\uncouple(G_\MANY,k)$, we denote by $\project$

We define the relation $\dominate_h$ on $\bigcup_n\AncPaths_G(n,k)$ as follows.
Let  $\pi=n_0\cdot a_1\cdot n_1\dots a_j\cdot n_j$ and
$\pi'=n_0'\cdot a_1'\cdot n_1'\dots a_h'\cdot n_h'$.
We have $\pi\dominate_h\pi'$ if the following two conditions are satisfied: 
(i) (i) $j\leq h$, 
(ii) for each $i\leq j$, $a_i=a_i'$ and $n_i\dominate_{G^\MANY}n_i'$, where $\dominate_{G^\MANY}$ is the maximal autoembedding of  $G^\MANY$.

 
The algorithm works in 5 stages. 
The algorithm first \emph{generalizes} the graph $G$, similarly to \simlearner, the uncoupled graph by assigning the arity \MANY to
every edge. 
After generalization, we \emph{uncouple} the input graph $G$ by creating copies of every non-literal node that has incoming
edges, one copy for each distinct  ancestor path (limiting the path to $k$ steps)\footnote{We could alternatively uncouple then generalize with the same result.}. Each copy has their own copies of the outgoing edges but receives only the incoming edges from nodes encoding the corresponding path. 
%Note that in the reduced graph $G^\MANY$ if a node has any incoming edges, they all have the same label and we refer to it as the \emph{parent  label}.
In the third stage, $\hybridlearner$ reduces the generalized graph $G^\MANY$ in a manner similar to $\simlearner$ but includes in the set of informative nodes Mx nodes that may be $\embedding$-dominated as long as they are not systematically dominated all along the ancestor path. 
The fourth step disconnects nodes in Mx from other nodes exactly as in \simlearner to reduce the graph. 
Finally, the arities are specialized using the induced embedding. This embedding is defined as follows.


Let $R$ denote the set of all $(\pi,\pi')\in N_{H_0}\times N_{H}$ such that the incoming edges of $\pi$ were redirected to $\pi'$ during $\mathsf{reduce}(H_0,\mathord{\dominate}_h)$. 
The induced embedding from $G$ to $H$ is the relation $\textit{induced-embedding}(G,H)=\{(\mathsf{last}(\pi),\pi')\mid (\pi,\pi')\in R\}$.



\begin{definition}
  A shape graph $H$ is \emph{k-ancestor-singular} iff there are no nodes $n\neq n'\in N_H$ and ancestor paths $\pi\in \AncPaths_H(n,k)$, $\pi'\in \AncPaths_H(n',k)$ such that $\pi\dominate_h\pi'$.
  % we do not impose uncoupling since that is not a property on the language and we don't really need it to clarify the following definition.
  By $\HybShExk{k}$ we denote the class of k-ancestor-singular shape graphs.  \qed
\end{definition}

For any schema in
$\HybShExk{k}(\ONE,\MANY)$ there exists a polynomially small characteristic
example as described below. 
\begin{definition}
  Fix $H\in\HybShExk{k}(\ONE,\MANY)$. Let $t\in N_H$ and  $\pi\in \AncPaths_H(t,k)$.
  A node $N\subseteq N_G$ of $G\in L(H)$
  \emph{characterises} $t\in N_H$ w.r.t. $\pi$ iff $n$ sim-characterises
  $t$ and $\pi\in \AncPaths_G(n,k)$.
\qed
\end{definition}
%\begin{definition}
%  Fix $H\in\HybShExk{k}(\ONE,\MANY)$. Let $t\in N_H$ and  $\pi\in \AncPaths_H(t,k)$.
%  A set of nodes $N\subseteq N_G$ of $G\in L(H)$
%  \emph{characterises} $t\in N_H$ w.r.t. $\pi$ iff for every $n\in N$, $n$ sim-characterises
%  $t$ and $\pi\in \AncPaths_G(n,k)$.
%\qed
%\end{definition}



A graph $G\in L(H)$ is a caracteristic example of $H$ if for every $t\in N_H$ and  $\pi\in \AncPaths_H(t,k)$, there is a set of nodes $N\subseteq N_G$ that characterizes $t$ w.r.t. $\pi$.

The definition is robust under extension i.e., for any $G'\in L(H)$ the graph $G_H\uplus G'$ is also
characteristic for $H$. We show that the algorithm
$\hybridlearner_{\{\ONE,\MANY\}}(G)$ returns $H$ for any $G$ that is
characteristic for $H$. 
Consequently, we show that $\hybridlearner_{\{\ONE,\MANY\}}$ is a sound and
complete inference algorithm for $\HybShExk{k}(\ONE,\MANY)$.
\begin{restatable}{theorem}{hybShExPolyLearnable}
  $\HybShExk{k}(\ONE,\MANY)$ is learnable in polynomial time and polynomial data
  from simple graphs.
\end{restatable}

\begin{proposition}
$\textit{induced-embedding}(G,H)$ is an embedding from $G$ to $H$. Furthermore, if $(n,\pi')\in \textit{induced-embedding}$ then 
there is a (suffix-)maximal ancestor path of $n$ that is dominated by $\pi'$. In other words, there is $i\leq k$ and $\pi=n_0a_0\dots n_i\in \AncPaths_G(n,k)$ such that $\pi \dominate_h\pi'$, and $i=k$ or $n_0$ has no parent in $G$.
\end{proposition}
\begin{proof}
The property is maintained through each step of $\mathsf{reduce}$. 
\end{proof}

\begin{proof}[Proof of the Theorem]
Let $G\in L(H)$ be a caracteristic example of $H$. Let $H'$ be the graph returned by $\hybridlearner_{\{\ONE,\MANY\}}$ on $G$. 
By construction, $H'$ is computed in polynomial time from $G$, and belongs to $\HybShExk{k}$.
We next prove that $L(H)=L(H')$.
Let $G'\in...$, and $n\in H'$.

\end{proof}



\iffalse
END OF PART CLEANED UP.
====================================================================================================
\color{gray}

$M$ contains $t\in N_{G^\MANY}$ iff for
every $s\in N_{G^\MANY}$ such that $t\embedding s$ we have that $s \embedding t$
or $t$ has an incoming edge with some label $a$ and $s$ has no incoming
$a$-edge.  Then, it removes all nodes not in $M$. In the
final stage the algorithm \emph{specializes} the reduced graph in precisely the
same way as \simlearner.

The algorithm constructs a schema that belongs to a class larger than
\SinShExZero and allows subtypes with different parent labels e.g.,
$\mathtt{e}\subseteq_{H_2}\mathtt{u}$. Formally,
\begin{definition}
  A shape graph $H$ is \emph{parent-singular} iff the equivalence classes of the
  maximal autoembedding of $H^\MANY$ has no two types with the same parent label.
  By $\HybShExk{k}$ we denote the class of parent-singular shape graphs.  \qed
\end{definition}
While the schema $H_0$ in Figure~\ref{fig:example} belongs to $\HybShExk{k}$,
the algorithm $\hybridlearner$ when presented with the graph $G_0$ outputs a
schema $H_2$ that is more specific: $H_2$ defines a flat hierarchy of
master-bugs that have been verified by an employee and that have a number of
related simple bugs that have not been verified. The main reason for this is
that the additional consideration of the parent label in the reduction stage
means that a stronger evidence is required to introduce recursion. Indeed, $G_0$
is not sufficiently informative of $H_0$ because it does not present any reason
why $H_2$ should not be a viable option. And since $H_2\subseteq H_0$, $H_2$ is
the preferred result of inference if we follow the \emph{mincon} principle. We
point out that by adding to $G_0$ a single edge
$(\mathtt{b_3},\mathtt{v},\mathtt{e}_1)$ we render the graph sufficiently
informative to make \hybridlearner return $H_0$. In fact, for any schema in
$\HybShExk{k}(\ONE,\MANY)$ there exists a polynomially small characteristic
example as described below. 
\begin{definition}
  Fix $H\in\HybShExk{k}(\ONE,\MANY)$. A set of nodes $N\in N_G$ of $G\in L(H)$
  \emph{parent-characterises} $t\in N_H$ iff every $n\in N$ sim-characterises
  $t$ and for every incoming edge of $t$ there is $n\in N$ that has an incoming
  edge with the same label. A graph $G$ is \emph{parent-characteristic} for $H$
  iff for every type $t$ of $H$ there is a set of nodes in $G$ that
  parent-characterises $t$. \qed
\end{definition}
Consequently, we show that \hybridlearner$_{\{\ONE,\MANY\}}$ is a sound and
complete inference algorithm for \HybShExk{k}(\ONE,\MANY).
\begin{restatable}{theorem}{hybShExPolyLearnable}
  $\HybShExk{k}(\ONE,\MANY)$ is learnable in polynomial time and polynomial data
  from simple graphs.
\end{restatable}
\color{black}

\fi

%%% Local Variables:
%%% mode: latex
%%% TeX-master: "paper"
%%% End:

